Using Large Language Models to Enrich the Documentation of Datasets for Machine Learning

Recent regulatory initiatives like the European AI Act and relevant voices in the Machine Learning (ML) community stress the need to describe datasets along several key dimensions for trustworthy AI, such as the provenance processes and social concerns. However, this information is typically presented as unstructured text in accompanying documentation, hampering their automated analysis and processing. In this work, we explore using large language models (LLM) and a set of prompting strategies to automatically extract these dimensions from documents and enrich the dataset description with them. Our approach could aid data publishers and practitioners in creating machine-readable documentation to improve the discoverability of their datasets, assess their compliance with current AI regulations, and improve the overall quality of ML models trained on them. In this paper, we evaluate the approach on 12 scientific dataset papers published in two scientific journals (Nature's Scientific Data and Elsevier's Data in Brief) using two different LLMs (GPT3.5 and Flan-UL2). Results show good accuracy with our prompt extraction strategies. Concrete results vary depending on the dimensions, but overall, GPT3.5 shows slightly better accuracy (81,21%) than FLAN-UL2 (69,13%) although it is more prone to hallucinations. We have released an open-source tool implementing our approach and a replication package, including the experiments' code and results, in an open-source repository.

==> sections/1.2objectives.tex <==
\section{Research objectives}
\label{sec:obj}

In this paper, we explore using LLM and several prompting strategies to automatically enrich the description of the machine learning dataset by extracting key information—categorized in a set of dimensions and sub-dimensions—from its raw documentation. We focused on the dimension demanded by the recent AI regulations and relevant voices in the ML community, and we were motivated by the recent apparition of structured formats that allow this dimension to be indexed by data search engines. %We believe our method could help create dataset machine-readable documentation, boost data discoverability, and aid in checking their legal compliance with emerging AI regulations.

%In this paper, we explore using LLM and several prompting strategies to automatically enrich the description of the machine learning dataset by extracting key information—categorized in a set of dimensions and sub-dimensions—from its raw documentation.

In summary, our research objective are as follows:

\begin{itemize}

\item \textbf{Research objective 1 (RO1)}: To explore the emerging LLM's suitability for extracting each of the desired dimensions from raw dataset documentation.

\item \textbf{Research objective 2 (RO2)}: To propose specific prompting strategies for extracting each dimension while avoiding hallucinations.

\item \textbf{Research objective 3 (RO3)}: To validate RO2 to real-world scientific data documentation

\item \textbf{Research objective 4 (RO4)}: To implement and release an open-source tool implementing RO2 and suited for RO3
   
\end{itemize}




